Permutation modules, Mackey functors, and Artin motives

We explain in detail the connections between the three concepts in the title, and we discuss how the `big' derived category of permutation modules introduced in arXiv:2009.14093 fits into the picture.

==> pmcs.tex <==


